Accelerated expansion as manifestation of gravity: when Dark Energy belongs to the left

In order to explain the Late-times accelerated expansion of the Universe we must appeal to some form of Dark Energy. In the standard model of cosmology, the latter is interpreted as a Cosmological Constant $\Lambda$. However, for a number of reasons, a Cosmological Constant is not completely satisfactory. In this thesis we study Dark Energy models of geometrical nature, and thus a manifestation of the underlying gravitational theory. In the first part of the thesis we will review the $\Lambda$CDM model and give a brief classification of the landscape of alternative Dark Energy candidates based on the Lovelock theorem. The second part of the thesis is instead devoted to the presentation of our main results on the topic of Dark Energy. To begin with, we will report our studies about nonlocal modifications of gravity involving the differential operator $\Box^{-1}R$, with emphasis on a specific model and on the common behavior shared by this and similar theories in the late stages of the evolution of the Universe. Then we introduce a novel class of modified gravity theories based on the anticurvature tensor $A^{\mu\nu}$ (the inverse of the Ricci tensor), and assess their capability as source of Dark Energy. Finally, we will discuss a type of drift effects which we predicted in the contest of Strong Gravitational Lensing, which could be employed both to study the effective equation of state of the Universe and to constrain violations of the Equivalence Principle.

==> abstract.tex <==

In order to explain the Late-times accelerated expansion of the Universe we must appeal to some form of Dark Energy. In the standard model of cosmology, the latter is interpreted as a Cosmological Constant $\Lambda$. However, for a number of reasons, a Cosmological Constant is not completely satisfactory. In this thesis we study Dark Energy models of geometrical nature, and thus a manifestation of the underlying gravitational theory. In the first part of the thesis we will review the $\Lambda$CDM model and give a brief classification of the landscape of alternative Dark Energy candidates based on the Lovelock theorem. The second part of the thesis is instead devoted to the presentation of our main results on the topic of Dark Energy.
To begin with, we will report our studies about nonlocal modifications of gravity involving the differential operator $\Box^{-1}R$, with emphasis on a specific model and on the common behavior shared by this and similar theories in the late stages of the evolution of the Universe. Then we introduce a novel class of modified gravity theories based on the anticurvature tensor $A^{\mu\nu}$ (the inverse of the Ricci tensor), and assess their capability as source of Dark Energy. Finally, we will discuss a type of drift effects which we predicted in the contest of Strong Gravitational Lensing, which could be employed both to study the effective equation of state of the Universe and to constrain violations of the Equivalence Principle.





==> acknowledgements.tex <==
\chapter*{Acknowledgments}

This work would not have been possible without the support and the help of a huge number of colleagues and professors who I had the pleasure and honour to met at the Federal University of Espirito Santo, and at the Institute for Theoretical Physics of Heidelberg.

In particular, I owe my deepest gratitude to Prof. Oliver Fabio Piattella, who did not just completely fulfilled his duties as a supervisor, but has also been the strongest influence and inspiration in my scientific training. It is possible that I have disappointed him as a student, but I hope I did not as a friend.
I want also to thank Prof. Luca Amendola for making possible my visiting stages in Heidelberg, and for letting me feel welcome and comfortable in its group.
Finally, I need to thank Doctors Tays Miranda and Emmanuel Frion, and M.Sc Giorgio Laverda, who actively contributed to part of the results I am going to present in this thesis, and even more importantly have been close to me when keeping going was not easy. 

The results presented in this thesis have been possible thanks to the financial support from the Coordenação de Aperfeiçoamento de Pessoal de Nível Superior - Brasil (CAPES) - Finance Code 001, and from the DAAD Co-financed Short-Term Research Grant Brazil, 2019 (57479964).



==> resumo.tex <==
Para explicar a expansão acelerada do Universo tardio é necessário recorrer a alguma forma de Energia Escura. No modelo padrão da cosmologia, ela é interpretada como uma constante cosmológica $\Lambda$. Porém, devido a várias razões, a constante cosmológica não é totalmente satisfatória. Nesta tese nós estudamos modelos alternativos onde a Energia escura é de natureza geométrica, e então é uma manifestação da teoria de gravitação subjacente. Na primeira parte da tese revisaremos o modelo $\Lambda$ e vamos dar uma breve classificação do panorama dos modelos alternativos de energia escura baseada no teorema de Lovelock. A segunda parte da tese, por outro lado, é dedicada a apresentação dos nossos resultados principais no tópico da Energia Escura. Para começar, nós iremos relatar nossos estudos sobre modificações não locais da gravitação que envolvem o operador diferencial $\Box^{-1}R$, com ênfase no modelo VAAS e no comportamento similar compartilhado por esta classe de teorias nos estágios finais da evolução do Universo. Em seguida, nós apresentamos uma nova classe de teorias de gravitação modificada 
que é baseada no tensor de anticurvatura $A_{\mu\nu}$, inverso do tensor de Ricci, e avaliamos o potencial dessas teorias como fonte de Energia Escura. Para concluirmos, discutiremos um tipo de efeitos de deriva que previmos no contexto de lentes gravitacionais fortes que poderiam ser empregados tanto para estudar a equação de estado efetiva do Universo quanto para restringir violações do princípio de equivalência.

